GeoGuesser Bench: Benchmarking Vision-Language Agents on Interactive Geolocation

Vision-language model (VLM) agents that act in the open world need two abilities: world knowledge to interpret what they see, and exploration to find what they cannot yet see. We study how agents combine the two through interactive visual geolocation. GeoGuesser Bench contains 282 tasks in an offline Street View environment where agents rotate, zoom, and move between real panoramas. Its three task types shift the balance from knowledge to exploration: agents (1) report the coordinates of their starting location, (2) name the enclosing street, city, state, or country, or (3) find, read, and count nearby objects. The coordinate tasks in (1) also include 42 real GeoGuessr World Championship rounds, whose expert guesses provide a human reference. We evaluate 23 VLMs: the best accuracy is 62.5% on place naming and 35.0% on object finding, and the best agent averages 4352.4 GeoGuessr points on the championship rounds, against 4770.3 for the better expert in each round. Beyond these headline numbers, world knowledge and exploration are only weakly correlated across models: agents that localize well do not necessarily explore well. To understand where agents fail, we categorize their errors into vision, navigation, and tool-use failures. Further ablations show that the strongest agents, such as Claude Opus 4.8, still perform well with limited views, while weaker agents degrade; customizing the environment thus adjusts task difficulty. The environment's verifiable rewards and restorable state also support training, and our Planner-Worker-Compressor harness cuts planner tokens by 57-61% by compacting the interaction history. We hope GeoGuesser Bench and its environment serve as a high-quality foundation for simulating real-world exploration at scale.

==> packages.tex <==
%%==================== Math ====================
\RequirePackage{amsmath}
\RequirePackage{amsthm}
\RequirePackage{amssymb}
\RequirePackage{mathtools}                % 必须在 amsmath 之后
\RequirePackage{bm}                       % commands.tex 的 \vzero 等依赖
\RequirePackage{mathpazo}

%%==================== 排版 / 字体 ====================
\RequirePackage{microtype}
\RequirePackage{anyfontsize}
\RequirePackage{titlesec}
\RequirePackage{tocloft}
% Headings and author metadata use the same Palatino family as the body.

%%==================== 颜色 ====================
\RequirePackage{xcolor}
\RequirePackage{colortbl}
%% ---- Google GM2 palette (single source; see CLAUDE.md "Color palette") ----
\definecolor{gblue}{HTML}{1A73E8}     % blue 600
\definecolor{gred}{HTML}{D93025}      % red 600
\definecolor{gyellow}{HTML}{E37400}   % yellow 900, the only Google yellow at 3:1 on white
\definecolor{ggreen}{HTML}{1E8E3E}    % green 600
\definecolor{gpurple}{HTML}{9334E6}   % purple 600
\definecolor{ggrey}{HTML}{5F6368}     % grey 700
\colorlet{linkcol}{gblue}

%%==================== 图与排版插入 ====================
\RequirePackage{graphicx}
\RequirePackage{wrapfig}
\RequirePackage{adjustbox}
\RequirePackage{tikz}                     % \circled 依赖

%%==================== Caption ====================
\RequirePackage[labelsep=colon]{caption}
\RequirePackage{subcaption}               % 必须在 caption 之后

%%==================== 表格 ====================
\RequirePackage{booktabs}
\RequirePackage{multirow}
\RequirePackage{tabularx}
\RequirePackage{makecell}

%%==================== 布局 ====================
\RequirePackage{geometry}
\RequirePackage{fancyhdr}
\RequirePackage{authblk}
\RequirePackage{enumitem}
\RequirePackage{tcolorbox}

%%==================== 工具 ====================
\RequirePackage{verbatim}
\RequirePackage{pifont}

%%==================== 算法 ====================
\RequirePackage[ruled,vlined,linesnumbered]{algorithm2e}
\RequirePackage{minted}                   % 需 -shell-escape

%%==================== Bib ====================
\RequirePackage[numbers,sort&compress]{natbib}

%%==================== Hyperref（必须最后加载）====================
\RequirePackage[colorlinks=true,allcolors=linkcol]{hyperref}
\RequirePackage[capitalize,noabbrev]{cleveref} % 必须在 hyperref 之后

